Exploring Popularity Bias in Session-based Recommendation

Existing work has revealed that large-scale offline evaluation of recommender systems for user-item interactions is prone to bias caused by the deployed system itself, as a form of closed loop feedback. Many adopt the \textit{propensity} concept to analyze or mitigate this empirical issue. In this work, we extend the analysis to session-based setup and adapted propensity calculation to the unique characteristics of session-based recommendation tasks. Our experiments incorporate neural models and KNN-based models, and cover both the music and the e-commerce domain. We study the distributions of propensity and different stratification techniques on different datasets and find that propensity-related traits are actually dataset-specific. We then leverage the effect of stratification and achieve promising results compared to the original models.

==> result1.tex <==
\begin{table*}[h]
\centering
% \scalebox{0.71}{
\begin{tabular}{lccc}
    \toprule  
    \textbf{Models} & HR@20 &   MRR@20\\
    \midrule  
    \textbf{GRU4REC} & & \\
    Ours  &  0.650  & 0.287  \\
    \cite{empirical} & 0.648 & 0.283\\
    \midrule
    % \textbf{V-SKNN} & & \\
    % Ours &  0.667  &  0.295  \\
    % \cite{empirical} & 0.651 & 0.287\\
    % \midrule
    \textbf{SKNN} & &\\
    Ours & 0.601 & 0.265 \\
    \cite{empirical} & 0.600 & 0.262\\
    \bottomrule 
\end{tabular}
% }
\vspace{-0.1cm}
\caption{RSC15 Dataset}
\label{tab:RSC15Rep}
\end{table*}

==> result2.tex <==
\begin{table*}[h]
\centering
% \scalebox{0.71}{
\begin{tabular}{lccc}
    \toprule  
    \textbf{Models} & HR@20 &   MRR@20\\
    \midrule  
    \textbf{GRU4REC} & & \\
    Ours  &  0.458  & 0.18  \\
    \cite{empirical} & 0.465 & 0.164\\
    \midrule
    \textbf{V-SKNN} & & \\
    Ours &  0.509 &  0.205 \\
    \cite{empirical} & 0.473 & 0.178\\
    \midrule
    \textbf{SKNN} & & \\
    Ours & 0.524 & 0.20\\
    \cite{empirical} & 0.475 & 0.1714\\
    \bottomrule 
\end{tabular}
% }
\vspace{-0.1cm}
\caption{Diginetica Dataset}
\label{tab:DigiRep}
\end{table*}

==> result3.tex <==
\begin{table*}[h]
\centering
% \scalebox{0.71}{
\begin{tabular}{lccc}
    \toprule  
    \textbf{Models} & HR@20 &   MRR@20\\
    \midrule  
    \textbf{GRU4REC} & &\\
    Ours &  0.569  & 0.33 \\
   \cite{empirical} & 0.567 & 0.324\\
    \midrule
    \textbf{V-SKNN} & & \\
    Ours &  0.572  &  0.348  \\
   \cite{empirical} & 0.575 & 0.340\\
    \midrule
    \textbf{SKNN} & & \\
    Ours & 0.595 & 0.346 \\
   \cite{empirical} & 0.579 & 0.337\\
    \bottomrule 
\end{tabular}
% }
\vspace{-0.1cm}
\caption{RetailRocket Dataset}
\label{tab:RetailRep}
\end{table*}

==> result4.tex <==
\begin{table*}[h]
\centering
% \scalebox{0.71}{
\begin{tabular}{lccc}
    \toprule  
    \textbf{Models} & HR@5 &   MRR@20 & NDCG@20\\
    \midrule  
    \textbf{GRU4REC} & & &\\
    Q1 &  0.402  & 0.299 & 0.397  \\
    Q2 & 0.8  & 0.519& 0.752 \\
    \midrule
    \textbf{V-SKNN} & & &\\
    Q1 &  0.419  &  0.309 & 0.409  \\
    Q2 & 0.95  &  0.558 & 0.817\\
    \midrule
    \textbf{SKNN} & & &\\
    Q1 & 0.422 & 0.312 & 0.409 \\
    Q2 & 0.925 & 0.604& 0.812\\
    \bottomrule 
\end{tabular}
% }
\vspace{-0.1cm}
\caption{Evaluation on stratified RetailRocket dataset}
\label{tab:RetailStrat}
\end{table*}

==> result5.tex <==
\begin{table*}[h]
\centering
% \scalebox{0.71}{
\begin{tabular}{lccc}
    \toprule  
    \textbf{Models} & HR@5 &   MRR@20 & NDCG@20\\
    \midrule  
    \textbf{GRU4REC} & & &\\
    Q1 & 0.25 & 0.166 & 0.272 \\
    Q2 & 0.59 & 0.35& 0.52\\
    \midrule
    \textbf{V-SKNN} & & &\\
    Q1 &  0.285  &  0.183 & 0.298  \\
    Q2 & 0.614 &  0.437 & 0.62\\
    \midrule
    \textbf{SKNN} & & &\\
    Q1 & 0.27 & 0.174 & 0.284 \\
    Q2 & 0.657 & 0.49& 0.65\\
    \bottomrule 
\end{tabular}
% }
\vspace{-0.1cm}
\caption{Evaluation on stratified Diginetica dataset}
\label{tab:DigiStrat}
\end{table*}

==> tab1.tex <==
\begin{table*}[h]
\centering
% \scalebox{0.71}{
\begin{tabular}{lccc}
    \toprule  
    \textbf{Strata} & Number of sessions & Number of distinct items &  Number of interactions  \\
    \midrule  
    Q1  &  15925  &  21138  &   76781  \\
    \midrule
    Q2  &  44  &  28  &  114  \\
    \bottomrule 
\end{tabular}
% }
\vspace{-0.1cm}
\caption{Strata statistics - Diginetica dataset}
\label{tab:sometable}
\end{table*}

==> tab2.tex <==
\begin{table*}[h]
\centering
% \scalebox{0.71}{
\begin{tabular}{lccc}
    \toprule  
    \textbf{Strata} & Number of sessions & Number of distinct items &  Number of interactions\\
    \midrule  
    Q1  &  2201  &  4244  &  7747  \\
    \midrule
    Q2  &  26  &  8  &  66  \\
    \bottomrule 
\end{tabular}
% }
\vspace{-0.1cm}
\caption{Strata statistics - Retailrocket dataset}
\label{tab:sometable}
\end{table*}
